Additive Gaussian Processes

We introduce a Gaussian process model of functions which are additive. An additive function is one which decomposes into a sum of low-dimensional functions, each depending on only a subset of the input variables. Additive GPs generalize both Generalized Additive Models, and the standard GP models which use squared-exponential kernels. Hyperparameter learning in this model can be seen as Bayesian Hierarchical Kernel Learning (HKL). We introduce an expressive but tractable parameterization of the kernel function, which allows efficient evaluation of all input interaction terms, whose number is exponential in the input dimension. The additional structure discoverable by this model results in increased interpretability, as well as state-of-the-art predictive power in regression tasks.

==> tables/nd_table.tex <==
% --- Automatically generated by resultsToLatex2.m ---
% Exported at 06-Apr-2011 14:10:51
\begin{table}[h!]
\caption{{\small
Dataset Statistics
}}
\label{tbl:Dataset Statistics}
\begin{center}
\begin{tabular}{l | r r}
Method & \rotatebox{90}{ N }  & \rotatebox{90}{ D }  \\ \hline
sanity easy

==> tables/r_sanity_easy_hypers_table.tex <==
% --- Automatically generated by hypers_to_latex.m ---
% Exported at 03-Jun-2011 00:23:44
\begin{table}[h]
\caption{{\small
Hyperparameters for sanity easy dataset.
}}
\label{tbl:sanity easy}
\begin{center}
\begin{tabular}{r | r r r}
Variable: & $x_1$  & $x_2$  & $x_3$  \\ \hline
Sq-exp lengthscale & $26253.73$  & $25456.47$  & $0.47$  \\ 
\hline
Additive lengthscale & $26254.84$  & $25470.23$  & $0.47$  \\
\hline
Order of interaction: & \nth{1} & \nth{2} & \nth{3} \\
Additive order variance & $0.0$\% & $0.1$\% & $99.9$\% \\ \hline
\end{tabular}
\end{center}
\end{table}
% End automatically generated LaTeX


==> tables/r_sanity_easy_hypers_table_grow.tex <==
% --- Automatically generated by hypers_to_latex.m ---
% Exported at 18-May-2011 13:44:56
\begin{table}[h]
\caption{{\small
Hyperparameters for r sanity easy dataset
}}
\label{tbl:r sanity easy}
\begin{center}
\begin{tabular}{l | r r r}
Variable: & $x_1$  & $x_2$  & $x_3$  \\ \hline
ARD Lengthscale & $1.20$  & $0.18$  & $4.43$  \\ 
\hline
ADD Lengthscale & $3.65$  & $0.23$  & $6.09$  \\
Order of Interaction: & \nth{1} & \nth{2} & \nth{3} \\
ADD Order Variance & $6.6$\% & $39.5$\% & $53.9$\% \\ \hline
\end{tabular}
\end{center}
\end{table}
% End automatically generated LaTeX


==> tables/r_sanity_hard_hypers_table.tex <==
% --- Automatically generated by hypers_to_latex.m ---
% Exported at 03-Jun-2011 00:23:44
\begin{table}[h]
\caption{{\small
Hyperparameters for sanity hard dataset.
}}
\label{tbl:sanity hard}
\begin{center}
\begin{tabular}{r | r r}
Variable: & $x_1$  & $x_2$  \\ \hline
Sq-exp lengthscale & $1.43$  & $0.19$  \\ 
\hline
Additive lengthscale & $1.43$  & $0.19$  \\
\hline
Order of interaction: & \nth{1} & \nth{2} \\
Additive order variance & $0.1$\% & $99.9$\% \\ \hline
\end{tabular}
\end{center}
\end{table}
% End automatically generated LaTeX


==> tables/r_sanity_hard_hypers_table_grow.tex <==
% --- Automatically generated by hypers_to_latex.m ---
% Exported at 18-May-2011 13:44:57
\begin{table}[h]
\caption{{\small
Hyperparameters for r sanity hard dataset
}}
\label{tbl:r sanity hard}
\begin{center}
\begin{tabular}{l | r r}
Variable: & $x_1$  & $x_2$  \\ \hline
ARD Lengthscale & $1538.91$  & $0.21$  \\ 
\hline
ADD Lengthscale & $119.83$  & $0.21$  \\
Order of Interaction: & \nth{1} & \nth{2} \\
ADD Order Variance & $0.0$\% & $100.0$\% \\ \hline
\end{tabular}
\end{center}
\end{table}
% End automatically generated LaTeX


==> tables/r_servo_hypers_table.tex <==
% --- Automatically generated by hypers_to_latex.m ---
% Exported at 03-Jun-2011 00:23:44
\begin{table}[h]
\caption{{\small
Hyperparameters for servo dataset.
}}
\label{tbl:servo}
\begin{center}
\begin{tabular}{r | r r r r}
Variable: & $x_1$  & $x_2$  & $x_3$  & $x_4$  \\ \hline
Sq-exp lengthscale & $1.46$  & $2.70$  & $1.13$  & $6.86$  \\ 
\hline
Additive lengthscale & $0.58$  & $0.80$  & $0.07$  & $2.57$  \\
\hline
Order of interaction: & \nth{1} & \nth{2} & \nth{3} & \nth{4} \\
Additive order variance & $58.7$\% & $27.4$\% & $0.0$\% & $13.9$\% \\ \hline
\end{tabular}
\end{center}
\end{table}
% End automatically generated LaTeX


==> tables/r_servo_hypers_table_grow.tex <==
% --- Automatically generated by hypers_to_latex.m ---
% Exported at 20-May-2011 20:59:40
\begin{table}[h]
\caption{{\small
Hyperparameters for r servo grow dataset
}}
\label{tbl:r servo grow}
\begin{center}
\begin{tabular}{l | r r r r}
Variable: & $x_1$  & $x_2$  & $x_3$  & $x_4$  \\ \hline
Sq-exp Lengthscale & $0.61$  & $0.88$  & $0.27$  & $3.33$  \\ 
\hline
Additive Lengthscale & $0.49$  & $0.69$  & $0.16$  & $2.46$  \\
\hline
Order of Interaction: & \nth{1} & \nth{2} & \nth{3} & \nth{4} \\
Additive Order Variance & $0.0$\% & $51.8$\% & $16.3$\% & $32.0$\% \\ \hline
\end{tabular}
\end{center}
\end{table}
% End automatically generated LaTeX


==> tables/rmse_table_all.tex <==
% --- Automatically generated by resultsToLatex3.m ---
% Exported at 04-May-2011 12:57:02
\begin{table}[h!]
\caption{{\small
Negative Log Likelihood
}}
\label{tbl:Negative Log Likelihood}
\begin{center}
\begin{tabular}{l | r r r r r r r r r r r r r r r r}
Method & \multicolumn{2}{c|}{ \rotatebox{0}{ lin model } } & \multicolumn{2}{c|}{ \rotatebox{0}{ gp ard } } & \multicolumn{2}{c|}{ \rotatebox{0}{ gp ard laplace } } & \multicolumn{2}{c|}{ \rotatebox{0}{ gp add 4 } } & \multicolumn{2}{c|}{ \rotatebox{0}{ gp add } } & \multicolumn{2}{c|}{ \rotatebox{0}{ gp add grow } } & \multicolumn{2}{c|}{ \rotatebox{0}{ gp add laplace 4 } } & \multicolumn{2}{c|}{ \rotatebox{0}{ gp add laplace } } & \multicolumn{2}{c|}{ \rotatebox{0}{ gp add laplace grow } }

==> tables/sanity_easy_hypers_table.tex <==
% --- Automatically generated by hypers_to_latex.m ---
% Exported at 12-May-2011 16:56:21
\begin{table}[h]
\caption{{\small
Hyperparameters for sanity easy dataset
}}
\label{tbl:sanity easy}
\begin{center}
\begin{tabular}{l | r r r}
Variable: & $x_1$  & $x_2$  & $x_3$  \\ \hline
ARD Lengthscale & $2514.48$  & $12980.31$  & $0.35$  \\ 
\hline
ADD Lengthscale & $871.23$  & $700.46$  & $0.45$  \\
ADD Variance & $0.87$ & $0.87$ & $1.08$ \\ \hline
Order of Interaction: & \nth{1} & \nth{2} & \nth{3} \\
ADD Order Variance & $2.9$\% & $0.0$\% & $97.1$\% \\ \hline
\end{tabular}
\end{center}
\end{table}
% End automatically generated LaTeX


==> tables/sanity_easy_hypers_table_grow.tex <==
% --- Automatically generated by hypers_to_latex.m ---
% Exported at 12-May-2011 16:56:21
\begin{table}[h]
\caption{{\small
Hyperparameters for sanity easy dataset
}}
\label{tbl:sanity easy}
\begin{center}
\begin{tabular}{l | r r r}
Variable: & $x_1$  & $x_2$  & $x_3$  \\ \hline
ARD Lengthscale & $2514.48$  & $12980.31$  & $0.35$  \\ 
\hline
ADD Lengthscale & $17.14$  & $0.05$  & $0.47$  \\
ADD Variance & $0.00$ & $0.00$ & $0.00$ \\ \hline
Order of Interaction: & \nth{1} & \nth{2} & \nth{3} \\
ADD Order Variance & $0.1$\% & $0.0$\% & $99.9$\% \\ \hline
\end{tabular}
\end{center}
\end{table}
% End automatically generated LaTeX


==> tables/sanity_hard_hypers_table.tex <==
% --- Automatically generated by hypers_to_latex.m ---
% Exported at 12-May-2011 16:56:21
\begin{table}[h]
\caption{{\small
Hyperparameters for sanity hard dataset
}}
\label{tbl:sanity hard}
\begin{center}
\begin{tabular}{l | r r}
Variable: & $x_1$  & $x_2$  \\ \hline
ARD Lengthscale & $0.47$  & $0.06$  \\ 
\hline
ADD Lengthscale & $0.47$  & $0.06$  \\
ADD Variance & $0.11$ & $1.06$ \\ \hline
Order of Interaction: & \nth{1} & \nth{2} \\
ADD Order Variance & $0.0$\% & $100.0$\% \\ \hline
\end{tabular}
\end{center}
\end{table}
% End automatically generated LaTeX


==> tables/sanity_hard_hypers_table_grow.tex <==
% --- Automatically generated by hypers_to_latex.m ---
% Exported at 12-May-2011 16:56:21
\begin{table}[h]
\caption{{\small
Hyperparameters for sanity hard dataset
}}
\label{tbl:sanity hard}
\begin{center}
\begin{tabular}{l | r r}
Variable: & $x_1$  & $x_2$  \\ \hline
ARD Lengthscale & $0.47$  & $0.06$  \\ 
\hline
ADD Lengthscale & $0.12$  & $0.02$  \\
ADD Variance & $0.00$ & $0.04$ \\ \hline
Order of Interaction: & \nth{1} & \nth{2} \\
ADD Order Variance & $100.0$\% & $0.0$\% \\ \hline
\end{tabular}
\end{center}
\end{table}
% End automatically generated LaTeX

